Harmless interpolation of noisy data in regression

A continuing mystery in understanding the empirical success of deep neural networks is their ability to achieve zero training error and generalize well, even when the training data is noisy and there are more parameters than data points. We investigate this overparameterized regime in linear regression, where all solutions that minimize training error interpolate the data, including noise. We characterize the fundamental generalization (mean-squared) error of any interpolating solution in the presence of noise, and show that this error decays to zero with the number of features. Thus, overparameterization can be explicitly beneficial in ensuring harmless interpolation of noise. We discuss two root causes for poor generalization that are complementary in nature -- signal "bleeding" into a large number of alias features, and overfitting of noise by parsimonious feature selectors. For the sparse linear model with noise, we provide a hybrid interpolating scheme that mitigates both these issues and achieves order-optimal MSE over all possible interpolating solutions.

==> commands_ISIT.tex <==
% \usepackage{fullpage}

\usepackage{epsf}
\usepackage{fancyheadings}
\usepackage{graphics}
\usepackage{graphicx,subfigure}
\usepackage{psfrag}

\usepackage{color}

\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}

\usepackage{accents}
\usepackage{listings}

\usepackage{caption}
%\usepackage{subcaption}
% *** SUBFIGURE PACKAGES ***
% \ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
% \else
%  \usepackage[caption=false,font=footnotesize]{subfig}
% \fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig
\usepackage[linesnumbered, ruled, vlined]{algorithm2e}

\usepackage[titletoc,toc,title]{appendix}




% \setlength{\textwidth}{\paperwidth}
% \addtolength{\textwidth}{-6cm}
% \setlength{\textheight}{\paperheight}
% \addtolength{\textheight}{-4cm}
% \addtolength{\textheight}{-1.1\headheight}
% \addtolength{\textheight}{-\headsep}
% \addtolength{\textheight}{-\footskip}
% \setlength{\oddsidemargin}{0.5cm}
% \setlength{\evensidemargin}{0.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS HERE

%%%%%%%
\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper
% \newtheorem{theorem}{Theorem}
% \newtheorem{remark}{Remark}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
% \newtheorem{fact}{Fact}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil 
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                } 
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother



%% COMMENTING commands

\long\def\comment#1{}



\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\vidyacomment}[1]{{\bf{{\blue{{Vidya --- #1}}}}}}
\newcommand{\anantcomment}[1]{{\bf{{\green{{Anant --- #1}}}}}}
\newcommand{\petercomment}[1]{{\bf{{\green{{Peter --- #1}}}}}}
\newcommand{\kailascomment}[1]{{\bf{{\green{{Kailas --- #1}}}}}}
\newcommand{\todo}[1]{{\bf{{\red{{TODO ---- #1}}}}}}




% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}


\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}

%Define horizontal and vertical bars
\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}
\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}



% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% Probability
\newcommand{\Exs}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

% Observations, dimension etc.
\newcommand{\numobs}{\ensuremath{n}}
\newcommand{\usedim}{\ensuremath{d}}



%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

% \DeclareMathOperator{\modd}{mod}
% \DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\var}{var}
% \DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\trace}{trace}
% \DeclareMathOperator{\abs}{abs}
% \DeclareMathOperator{\floor}{floor}
% \DeclareMathOperator{\vol}{vol}
% \DeclareMathOperator{\child}{child}
% \DeclareMathOperator{\parent}{parent}
% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\toeplitz}{toeplitz}


% 
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{Ber}}}

\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}

\newcommand{\Sspace}{\ensuremath{\mathcal{S}}}
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}


\newcommand{\Uspace}{\ensuremath{\mathcal{U}}}
\newcommand{\Dspace}{\ensuremath{\mathcal{D}}}
\newcommand{\Tspace}{\ensuremath{\mathcal{T}}}
\newcommand{\Mspace}{\ensuremath{\mathcal{M}}}

\newcommand{\off}{\ensuremath{\mathsf{off}}}
\newcommand{\boldf}{\ensuremath{\mathbf{f}}}
\newcommand{\lvec}{\ensuremath{\mathbf{l}}}
\newcommand{\Lvec}{\ensuremath{\mathbf{L}}}

\newcommand{\xvec}{\ensuremath{\mathbf{x}}}
\newcommand{\vvec}{\ensuremath{\mathbf{v}}}
\newcommand{\Xvec}{\ensuremath{\mathbf{X}}}
\newcommand{\Yvec}{\ensuremath{\mathbf{Y}}}
\newcommand{\Wvec}{\ensuremath{\mathbf{W}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\newcommand{\EE}{\ensuremath{\mathbb{E}}}
% Basic statistics notation
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
\newcommand{\alphastar}{\ensuremath{\alpha^*}}
\newcommand{\betastar}{\ensuremath{\beta^*}}
\newcommand{\gammastar}{\ensuremath{\gamma^*}}

\newcommand{\Thetastar}{\ensuremath{\Theta^*}}
\newcommand{\Sigmastar}{\ensuremath{\Sigma^*}}
\newcommand{\Mstar}{\ensuremath{M^*}}

%Best action
\newcommand{\kstar}{\ensuremath{k^*}}
% Estimate one
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\Thetahat}{\ensuremath{\widehat{\Theta}}}
\newcommand{\Sigmahat}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\gammahat}{\ensuremath{\widehat{\gamma}}}
\newcommand{\Deltahat}{\ensuremath{\widehat{\Delta}}}
\newcommand{\alphahat}{\ensuremath{\widehat{\alpha}}}
\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\Phat}{\ensuremath{\widehat{P}}}
\newcommand{\pistar}{\ensuremath{\pi^*}}
\newcommand{\xhat}{\ensuremath{\widehat{x}}}
% Estimate two
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

\newcommand{\testerr}{\ensuremath{\mathcal{E}_{\mathsf{test}}}}


\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}

\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}

%Algorithm notation
\newcommand{\alg}[1]{\textsc{#1}}
\newcommand{\Oh}{\ensuremath{\mathcal{O}}}

%Problem-specific notation
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\cone}{\ensuremath{\mathbb{C}}}

\newcommand{\ltwoball}{\ensuremath{\mathbb{B}^{p-1}_2}}
\newcommand{\lzeroball}{\ensuremath{\mathbb{B}^{p-1}f_0}}

\newcommand{\gprop}{\ensuremath{g_{\mathsf{prop}}}}
\newcommand{\gunif}{\ensuremath{g_{\mathsf{unif}}}}
\newcommand{\thigh}{\ensuremath{t_{\mathsf{high}}}}
\newcommand{\tlow}{\ensuremath{t_{\mathsf{low}}}}
\newcommand{\wtree}{\ensuremath{w^{(\mathsf{tree})}}}
\newcommand{\ltree}{\ensuremath{l^{(\mathsf{tree})}}}
\newcommand{\Ltree}{\ensuremath{L^{(\mathsf{tree})}}}
\newcommand{\lvectree}{\ensuremath{\lvec^{(\mathsf{tree})}}}
\newcommand{\Lvectree}{\ensuremath{\Lvec^{(\mathsf{tree})}}}
\newcommand{\wvectree}{\ensuremath{\wvec^{(\mathsf{tree})}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%FIGURES
% QUICK FIGURE
% Usage:
%{fig:my_figure}{Caption}{Figures/placeholder.jpg}{0.5\textwidth}
\newcommand{\quickfigure}[4]{
  \begin{figure}[htbp]
  \centering
  \includegraphics[width=#4]{#3}
  \caption{#2}
  \label{#1}
  \end{figure}
}

\newcommand{\quadfigureinterior}[9]{
 \subfigure[#2]{
  \includegraphics[width=#1]{#3}
   }
 \subfigure[#4]{
  \includegraphics[width=#1]{#5}
   }
 \subfigure[#6]{
  \includegraphics[width=#1]{#7}
   }
 \subfigure[#8]{
  \includegraphics[width=#1]{#9}
   }
}

\newcommand{\quadfigureexterior}[3]{
\begin{figure}[htbp]
 %\centering
 #3
 \caption{#2}
 \label{#1}
\end{figure}
}

% Usage:
%\multifigureexterior{fig:myfigure}{Overall caption}{
%  \subfig{\halftextfigwidth}{Caption}{Figures/placeholder.jpg}
%  \subfig{\halftextfigwidth}{Caption}{Figures/placeholder.jpg}
%}
\newcommand{\multifigureexterior}[3]{\quadfigureexterior{#1}{#2}{#3}}

% Usage:
%\subfig{\halftextfigwidth}{Caption}{Figures/placeholder.jpg}
%\subfigl{\halftextfigwidth}{fig:myfigure}{Caption}{Figures/placeholder.jpg}
\newcommand{\subfigl}[4]{\subfigure[#3]{\includegraphics[width=#1]{#4} \label{#2}}}
\newcommand{\subfig}[3]{\subfigl{#1}{}{#2}{#3}}


%Mathsf notations
\newcommand{\supp}{\mathsf{supp}}
\newcommand{\Atrain}{A_{\mathsf{train}}}
\newcommand{\Btrain}{B_{\mathsf{train}}}
\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Ytrain}{\mathbf{Y}_{\mathsf{train}}}
\newcommand{\Wtrain}{\mathbf{W}_{\mathsf{train}}}
\newcommand{\bvec}{\mathbf{b}}
\newcommand{\avec}{\mathbf{a}}
